AnTenA: Actionable and Explainable Tensor Analysis System with Large Language Models

Accurately explaining hidden patterns in multi-aspect data has typically been done by leveraging labels and/or accompanying auxiliary metadata. However, labels and auxiliary data may be inaccurate (e.g. nonstandard, inconsistent), insufficient (e.g. static tabular metadata for time-dependent recordings), or unavailable. % We propose \fullmethod (\method), which leverages the knowledge of large language models (LLMs) to explain the hidden patterns in human narratives. \method uses task-agnostic and task-specific prompts to explain extracted co-clustered latent patterns from tensor decomposition. To evaluate these explanations, we test the LLMs on forward and backward inference tasks. % Our demo system is available at https://github.com/dawonahn/ECML_PKDD_AnTenA.

==> 050related.tex <==
% \subsection{Explainable AI}
% \audrey{Figure~\ref{fig:tensor_analysis}.2 shows two forms of explanations that can accompany the results of tensor decomposition on the MovieLens dataset.}
% The first uses the dataset metadata only and the top four movies returned by the decomposition.
% The second explanation is a tabular output from ChatGPT's XXX model (accessed June 2025) after being given the following prompt: \\
% \texttt{"Input Description: \\
% 1. Hidden patterns are represented as rank-one components of (movie, user, and time) extracted from CANDECOMP/PARAFAC decomposition.\\
% 2. Top-K rank-one components are stored in a dictionary with keys as hidden pattern indices. \\
% Task description: \\
% 1. Evaluate the quality of patterns (movie-user-time) by comparing all patterns in terms of Quality (do the top movies/users/times make sense together (i.e., are they thematically consistent)) and Interpretability (overlap between patterns lowers overall uniqueness). \\
% 2. What is the main theme/genre of each pattern?\
% 3. Return a summary table with answers to the questions above with the columns (Pattern, Theme/Genre, Quality, Interpretability, Recommendation) \\
% 4. Return the stat of quality of patterns in the format:\
% Pattern quality (high=3, moderate-high=2.5, moderate = 2, low-moderate=1.5, low = 1): pattern\_quality\_score, interpretability\_score (mean of evaluation). \\
% 5. Return only summary table and quality scores."}
% [Insert output from LLM here.]

% \noindent \textbf{Neural Tensor Models.}
% CANDECOMP/PARAFAC (CP)~\cite{kolda2009tensor} is widely used due to its simplicity and interpretability.
% However, it is limited to multi-linear operations, and often fails to fit tensors non-linear latent structures. 
% \textbf{Neural Tensor Models} like NeAT~\cite{ahn2024neural} have been  proposed to maintain the CPD structure, while capturing non-linear latent patterns. Our proposed framework uses LLMs as a \textbf{tensor analysis system} to interpret components decomposed by these neural tensor models into natural language bridges the gap between interpretable-by-design outputs into actionable insight.
% The latent components from tensor models are not directly human-interpretable.
% However, they only use metadata to explain tensor decomposition results from \textit{classical} tensor decomposition methods.
% Several tensor analysis tools have been proposed~\cite{park2016bigtensor,ahn2020gtensor} to expedite the large-scale tensor decomposition speed by using heterogeneous systems and distributed system. % -- I might propose removing it unless you want to argue claims to speed and scalability compared to other methods
 % it might be helpful to describe 1) what their output is and 2) why that LLM output is less helpful to humans than the natural language version you propose here in this paper 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CANDECOMP/PARAFAC (CP)~\cite{kolda2009tensor} and Tucker decomposition~\cite{} are conventional tensor models to analyze tensors.
% % Applications
% % Development of model on specific property.
% Traditionally, CPD and Tucker decomposition successfully fit low-rank linear structures, but  often fail to fit tensors including non-linear latent structures~\cite{liu2019costco}.
% Numerous methods have been developed to replace multi-linear operations with neural networks to capture complex structures and show remarkable performance in tensor completion~\cite{he2017neural,liu2018neuralcp,liu2019costco,chen2020neural,tillinghast2020probabilistic,qian2022julia,ahn2024neural}.
% %
% While these neural tensor models are accurate, they no longer have the same interpretable-by-design characteristic of the classic CPD and Tucker decompositions.
% Neural tensor models' networks entangle latent components, making it challenging to interpret the decomposition results. 
% NeAT~\cite{ahn2024neural} maintains the CPD structure, applying shallow MLPs to each component to capture latent patterns while preserving their intuitive explainability. 
% % Note, if this work is being positioned to sit on top of explainable decomposition methods like NeAT (or even CPD or Tucker for that matter), then adding a sentence about, "However, NeAt, CPD, and Tucker decomposition steps stop at producing interpretable components, and these components are not directly human-interpretable. Our proposed framework using LLMs to interpret these components into natural language bridges the gap between interpretable-by-design outputs into actionable insight."
% %
% Several tensor analysis tools have been proposed 
% ~\cite{park2016bigtensor,ahn2020gtensor} to expedite the large-scale tensor decomposition speed by using heterogeneous systems and distributed system. % Not sure where speed and scalability are coming into the thesis -- is this another challenge that this proposed method must overcome? - Audrey
% % These two papers are existing demo systems for tensor analysis. I just wanted to explain that tensor analysis demo system focusing on explainability do not exist before. 
% % To explain this, I wrote down their works' purpose for demo system, which is speed or scalibility while ours focus on accuracy and explainiability. 
% % Basicially, the differences between our work and existing works... Let me now if still something is not clear!
% %
% These tensor analysis systems have two limitations: 
% 1) it is challenging for classical multi-linear tensor models to capture complex patterns in real-world tensors, and 2) tensor analysis results are difficult to directly understand.
